Text-Guided Mask-free Local Image Retouching

In the realm of multi-modality, text-guided image retouching techniques emerged with the advent of deep learning. Most currently available text-guided methods, however, rely on object-level supervision to constrain the region that may be modified. This not only makes it more challenging to develop these algorithms, but it also limits how widely deep learning can be used for image retouching. In this paper, we offer a text-guided mask-free image retouching approach that yields consistent results to address this concern. In order to perform image retouching without mask supervision, our technique can construct plausible and edge-sharp masks based on the text for each object in the image. Extensive experiments have shown that our method can produce high-quality, accurate images based on spoken language. The source code will be released soon.

==> Figures/complex_mask.tex <==
\begin{figure}[!htb]
\centering
\includegraphics[width=\linewidth]{images/ComplexMask.pdf}
\caption{Mask generation.}
\label{fig:MaskGeneration}
\end{figure}

==> Tables/Validate_Proposals.tex <==
% \begin{table}[!htb]
% \centering
% \caption{In order to measure the impact of the different number of proposal settings on the final result, experiments were carried out on different numbers of proposals}  % 表格标题
% \label{Proposals}  % 用于索引表格的标签
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|c|c|c|c|c|c}
% \hline
% Dataset                   & Proposals & SSIM($\uparrow$) & PSNR($\uparrow$) & FID($\downarrow$) & MES($\downarrow$) & LPIPS($\downarrow$) \\ \hline
% \multirow{4}{*}{ITMSCOCO} & 1         &   0.7042   &   17.7389   &   16.7268  &  0.0218  &  0.2673  \\ \cline{2-7} 
%                           & 2         &   0.7101   &   17.7829   &   14.8556  &  0.0198  &  0.2614  \\ \cline{2-7} 
%                           & 3         &   0.7119   &   17.7837   &   14.5479  &  0.0193  &  0.2602  \\ \cline{2-7} 
%                           & 4         &   0.7125   &   17.8141   &   14.5512  &  0.0190  &  0.2605  \\ \hline
% \multirow{4}{*}{ITFliker} & 1         &   0.6840   &   17.3170   &   14.4946  &  0.0227  &  0.2624  \\ \cline{2-7} 
%                           & 2         &   0.6907   &   17.3861   &   12.4683  &  0.0208  &  0.2556  \\ \cline{2-7} 
%                           & 3         &   0.6922   &   17.4282   &   12.2894  &  0.0205  &  0.2547  \\ \cline{2-7} 
%                           & 4         &   0.6923   &   17.4375   &   12.0330  &  0.0203  &  0.2541  \\ \hline
% \end{tabular}%
% }
% \end{table}
\begin{table}[!htb]
\centering
\caption{In order to measure the impact of the different number of proposal settings on the final result, experiments were carried out on different numbers of proposals}  % 表格标题
\label{Proposals}  % 用于索引表格的标签
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\hline
 Proposals & SSIM($\uparrow$) & PSNR($\uparrow$) & FID($\downarrow$) & MES($\downarrow$) & LPIPS($\downarrow$) \\ \hline
% \multirow{4}{*}{ITMSCOCO} & 1         &   0.7042   &   17.7389   &   16.7268  &  0.0218  &  0.2673  \\ \cline{2-7} 
%                           & 2         &   0.7101   &   17.7829   &   14.8556  &  0.0198  &  0.2614  \\ \cline{2-7} 
%                           & 3         &   0.7119   &   17.7837   &   14.5479  &  0.0193  &  0.2602  \\ \cline{2-7} 
%                           & 4         &   0.7125   &   17.8141   &   14.5512  &  0.0190  &  0.2605  \\ \hline
1         &   0.6840   &   17.3170   &   14.4946  &  0.0227  &  0.2624  \\ \cline{1-6} 
2         &   0.6907   &   17.3861   &   12.4683  &  0.0208  &  0.2556  \\ \cline{1-6} 
3         &   0.6922   &   17.4282   &   12.2894  &  0.0205  &  0.2547  \\ \cline{1-6} 
4         &   0.6923   &   17.4375   &   12.0330  &  0.0203  &  0.2541  \\ \hline
\end{tabular}%
}
\end{table}

==> Tables/Validate_Timesteps.tex <==
% \begin{table}[!htb]
% \centering
% \caption{standard table}  % 表格标题
% \label{tab:timesteps}  % 用于索引表格的标签
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|c|c|c|c|c|c}
% \hline
% Dataset                   & Timesteps & SSIM($\uparrow$) & PSNR($\uparrow$) & FID($\downarrow$) & MES($\downarrow$) & LPIPS($\downarrow$)\\ \hline
% \multirow{4}{*}{ITMSCOCO} & 20        &  0.6954  &  17.7541    &  11.3578   & 0.01890    & 0.2499\\ \cline{2-7}
%                           & 50        &  0.7122  &  17.8983    &  14.4055   & 0.01874    & 0.2530\\ \cline{2-7} 
%                           & 100       &  0.7126  &  17.8266    &  14.4801   & 0.01893    & \\ \cline{2-7} 
%                           & 200       &  0.7125  &  17.8141    &   14.5512  &  0.0190  &   0.2605  \\ \cline{1-7} 
% \multirow{3}{*}{ITFliker} & 50        &  0.6923  &  17.5719    &  12.0685   &  0.0197  & \\ \cline{2-7} 
%                           & 100       &  0.6931  &  17.4897    &  12.0676   &  0.0201  & \\ \cline{2-7} 
%                           & 200       &  0.6923  &  17.4375    &   12.0330   &   0.0203  &   0.2541 \\ \hline
% \end{tabular}%
% }
% \end{table}
